gZCCL: Compression-Accelerated Collective Communication Framework for GPU Clusters

GPU-aware collective communication has become a major bottleneck for modern computing platforms as GPU computing power rapidly rises. A traditional approach is to directly integrate lossy compression into GPU-aware collectives, which can lead to serious performance issues such as underutilized GPU devices and uncontrolled data distortion. In order to address these issues, in this paper, we propose gZCCL, a first-ever general framework that designs and optimizes GPU-aware, compression-enabled collectives with an accuracy-aware design to control error propagation. To validate our framework, we evaluate the performance on up to 512 NVIDIA A100 GPUs with real-world applications and datasets. Experimental results demonstrate that our gZCCL-accelerated collectives, including both collective computation (Allreduce) and collective data movement (Scatter), can outperform NCCL as well as Cray MPI by up to 4.5X and 28.7X, respectively. Furthermore, our accuracy evaluation with an image-stacking application confirms the high reconstructed data quality of our accuracy-aware framework.

==> Makefile <==
#
# $Id: Makefile 279 2008-01-27 16:19:38Z balaji $
#
# Copyright (C) 2006-2007, University of Chicago. All rights reserved.
#

HEADER = ACMmain
PICS = picture
BIB = bib
TEX = tex

TARGETS: $(HEADER).pdf
.PHONY: all clean $(HEADER).pdf

tex_files = $(shell find $(TEX) -name '*.tex' -print)
bib_files = $(shell find $(BIB) -name '*.bib' -print)
pic_files = $(shell find $(PICS) \
		\( -name '*.eps' -print \) -or \( -name '*.epsi' -print \) \
		-or \( -name '*.ps' -print \) -or \( -name '*.png' -print \) \
		-or \( -name '*.fig' -print \) -or \( -name '*.pdf' -print \) \
	)

$(HEADER).pdf: $(HEADER).tex $(tex_files) $(bib_files) $(pic_files)
	@if test "`which rubber`" != "" ; then \
		TEXMFOUTPUT=`pwd` rubber -c 'setlist arguments -shell-escape' --unsafe -d -f $(HEADER) ; \
	else \
		pdflatex -shell-escape $(HEADER) | tee latex.out ; \
		if grep -q 'Citation.*undefined' latex.out; then \
			bibtex $(HEADER); \
			touch .rebuild; \
		fi ; \
		while [ -f .rebuild -o \
			-n "`grep '.*Rerun' latex.out`" ]; do \
			rm -f .rebuild; \
			pdflatex -shell-escape $(HEADER) | tee latex.out; \
		done ; \
		rm -f latex.out ; \
	fi

clean:
	@if test "`which rubber`" != "" ; then \
		rubber -c 'setlist arguments -shell-escape' -d --clean $(HEADER) ; \
	else \
		find . \( -name '*.blg' -print \) -or \( -name '*.aux' -print \) -or \
			\( -name '*.bbl' -print \) -or \( -name '*~' -print \) -or \
			\( -name '*.lof' -print \) -or \( -name '*.lot' -print \) -or \
			\( -name '*.toc' -print \) -or \( -name '*.fdb_latexmk' -print \) -or \
			\( -name '*.fls' -print \) -or \( -name '*.synctex.gz' -print \) | xargs rm -f; \
		rm -f $(HEADER).dvi $(HEADER).log $(HEADER).ps $(HEADER).pdf $(HEADER).out \
			_region_* TAGS ; \
	fi


==> related.tex <==
\section{Related Work}\label{related}

